Complex-valued convolutional neural network classification of hand gesture from radar images

Hand gesture recognition systems have yielded many exciting advancements in the last decade and become more popular in HCI (human-computer interaction) with several application areas, which spans from safety and security applications to automotive field. Various deep neural network architectures have already been inspected for hand gesture recognition systems, including multi-layer perceptron (MLP), convolutional neural network (CNN), recurrent neural network (RNN) and a cascade of the last two architectures known as CNN-RNN. However, a major problem still exists, which is most of the existing ML algorithms are designed and developed the building blocks and techniques for real-valued (RV). Researchers applied various RV techniques on the complex-valued (CV) radar images, such as converting a CV optimisation problem into a RV one, by splitting the complex numbers into their real and imaginary parts. However, the major disadvantage of this method is that the resulting algorithm will double the network dimensions. Recent work on RNNs and other fundamental theoretical analysis suggest that CV numbers have a richer representational capacity, but due to the absence of the building blocks required to design such models, the performance of CV networks are marginalised. In this report, we propose a fully CV-CNN, including all building blocks, forward and backward operations, and derivatives all in complex domain. We explore our proposed classification model on two sets of CV hand gesture radar images in comparison with the equivalent RV model. In chapter five, we propose a CV-forward residual network, for the purpose of binary classification of the two sets of CV hand gesture radar datasets and compare its performance with our proposed CV-CNN and a baseline CV-forward CNN.

==> y4realdataapp.tex <==
\chapter{Real-value Dataset}




\section{Real-value Dataset}
\cite{complexcnn} designed and implemented a complex-forward residual network and they only test the performance of the network with real-value datasets. In order to create a comparison we experiment training all three fully complex CNN, complex-forward residual and the complex-forward CNN with two class of Cifar-$10$. We copy the real component to create the imaginary component for the real-value Cifar-$10$ dataset, therefore  the sample dimension is doubles from$32\times32\times3$.  

\subsection{Cifar-$10$ class dataset}


The Canadian Institute for Advanced Research (Cifar) is a Canadian-based global research organisation that brings together teams of top researchers from around the world to address important and complex questions. The Cifar-$10$ dataset is one of the most widely used datasets for machine learning research~\cite{ciften}. Cifar-$10$ is currently one of the most widely used datasets in machine learning and serves as a test ground for many computer vision methods. A concrete measure of popularity is the fact that Cifar-10 was the second most common dataset in NIPS 2017 (after MNIST) ~\cite{cifhamner}~\cite{cifgen}.

The CIFAR-$10$ dataset consists of $60000$ $32\times32\times 3$colour images in $10$ classes, with $6000$ images per class. There are $50000$ training images and $10000$ test images.

The dataset is divided into five training batches and one test batch, each with $10000$ images. The test batch contains exactly $1000$ randomly-selected images from each class. The training batches contain the remaining images in random order, but some training batches may contain more images from one class than another. Between them, the training batches contain exactly $5000$ images from each class.

The Cifar-$10$ dataset consists of $10$ classes of airplane, automobile, bird, cat, deer, dog, frog, horse, ship and truck~\fig{cifar}

We have used $2$ random classes of the Cifar-$10$ dataset, so that we have got $10000$ training and $2000$ test samples for the binary classification experiments. ~\fig{cifar} illustrates $10$ sample images of each class.


\begin{figure}
\centering\includegraphics[scale=0.8]{cifar10.png}
\caption{Cifar-10 classes samples}
\label{fig:cifar}
\end{figure}


\subsection{Our Real-value Dataset}

We have randomly selected $2$ classes of Cifar-10 datasets as our real-value dataset, which consist of $10000$ training and $2000$ test samples in total. In order to test our complex network architectures we have added a copy of the real-value samples to create the imaginary value for each sample, therefore we create a new complex-value alike test and training datasets that each sample dimensions are $32\times32\times6$   instead of $60000$ $32\times32$ in the original Cifar-10 dataset. 



However, \cite{complexnn} that creates the imaginary part for each sample by applying two layer of batch normalisation, activation function and a $2$D convolution on each sample of the dataset and apply the imaginary part alongside the real part of each sample to the residual network with complex blocks.  




\section{Real-value Dataset Results}

\subsection{Complex-forward Residual Network}
This section displays some experiment result of training the complex-forward residual network with $2$ classes of Cifar-$10$.
\begin{figure}
\centering\includegraphics[scale=0.9]{cifarresbigtable.png}
\caption{Cifar$10$ dataset Complex-forward Residual architecture  }
\label{fig:cifarresone}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarressmalltable.png}
\caption{Cifar-$10$ dataset Complex-forward Residual parameters setting }
\label{fig:cifarrestwo}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarresgraph.png}
\caption{Cifar-$10$ dataset Complex-forward Residual accuracy per epoch (for Figure~\figg{cifarresone}, \figg{cifarrestwo} setting)  }
\label{fig:cifarresthree}
\end{figure}

\subsection{Complex-forward CNN Network}

This section displays some experiment result of training the complex-forward CNN network with $2$ classes of Cifar-$10$.
\begin{figure}
\centering\includegraphics[scale=0.9]{cifarconv1bigtable.png}
\caption{Cifar$10$ dataset Complex-forward CNN architecture  }
\label{fig:cifarconvone}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarconv1smalltable.png}
\caption{Cifar-$10$ dataset Complex-forward CNN parameters setting }
\label{fig:cifarconvtwo}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarconv1graph.png}
\caption{Cifar-$10$ dataset Complex-forward CNN accuracy per epoch (for Figure~\figg{cifarconvone}, \figg{cifarconvtwo} setting)  }
\label{fig:cifarconvthree}
\end{figure}




\subsection{Complex CNN Network}

This section displays some experiment result of training the fully complex CNN network with $2$ classes of Cifar-$10$.

\begin{figure}
\centering\includegraphics[scale=0.9]{cifarmycode1bigtable.png}
\caption{Cifar$10$ dataset Complex CNN architecture  }
\label{fig:cifarmyone}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarmycode1smalltable.png}
\caption{Cifar-$10$ dataset Complex CNN parameters setting }
\label{fig:cifarmytwo}
\end{figure}


\begin{figure}
\centering\includegraphics[scale=0.9]{cifarmycode1graph.png}
\caption{Cifar-$10$ dataset Complex CNN accuracy per epoch (for Figure~\figg{cifarmyone}, \figg{cifarmytwo} setting)  }
\label{fig:cifarmythree}
\end{figure}



==> year4dataset.tex <==
\chapter{ Datasets}


\section{Complex-value Dataset} 
\subsection{DopNet}


DopNet is a large Radar database organised in a hierarchy, each node in DopNet represents the data of one person which is divided into different gestures recorded from that person. The data is measured with FMCW(Frequency Modulated Continuous Wave) and CW(Continuous Wave) Radars. DopNet‘s structure makes it a useful tool for Machine Learning Gesture Recognition, software and Image Processing for the spectrograms. The shared data was generated by Dr. Matthew Ritchie (University College London (UCL), London, United Kingdom) and Richard Capraru (Nanyang Technological University (NTU) and Singapore Agency for Science, Technology and Research (A*STAR), Singapore) within the UCL Radar Research Group in collaboration with Dr. Francesco Fioranelli (Delft University of Technology (TU Delft), Delft, Netherlands). Furthermore, it started as a Laidlaw Scholarship project.~\cite{dopnet}



FMCW Radar system is a special type of radar system that measures both velocity and distance of a moving object. This is achieved by continuously transmits a Chirp, which is a signal that increases (up-chirp) or decreases (down-chirp) its frequency linearly with time, This is then mixed with the received signal in order to obtain the range (Doppler) of a target. FMCW radar system measures the frequency difference between the transmitted and received echo signal for calculating the distance, and it also measures the Doppler frequency (due to the Doppler effect) for calculating the speed of the object. 


Radar sensors have previously been successfully used to classify different actions such as walking, carrying an item, discriminating between people and animals gaits or drones and bird targets~\cite{fiorone}~\cite{fiortwo}~\cite{fiorthree}~\cite{tah}. All of this analysis used the phenomenon called Micro-Doppler which is the additional movements a target has on top of its bulk velocity. For example, a person may walk forwards at $3$ m/s but as they move at this speed their arms and legs oscillate back and forth. This movement creates a signature which was coined as Micro-Doppler by researcher ~\cite{vchen}.



\begin{figure}
\centering\includegraphics[scale=0.8]{gesturepic.png}
\caption{ Wave, Pinch, Click, Swip gestures ~ \cite{dopnet}}
\label{fig:gestu}
\end{figure}




 A database of gestures has been created which includes signals from $4$ different types Wave, Pinch, Click, Swipe for person A, B, C,D, E and F~\fig{gestu}. The data itself has been pre-processed so that the signatures have been cut into individual actions from a long data stream, filtered to enhance the desired components and processed to produce the Doppler vs. time-domain data. The data is then stored in this format in order for it to be read in, features to be extracted and the classification process to be performed~\cite{dopnet}.
The data generated for this classification challenge was created using an Ancortek $24$ GHz FMCW radar a $750$ MHz bandwidth, more details about the radar system can be seen in the table ~\tbl{gest}. 

\begin{table}
\centering\scalebox{0.9}{  
 \begin{tabular}{|c|c|r}
  \hline
  \hline
  Parameter & Value \\
  \hline
  \hline
  Frequency & $24$ GHz  \\
  \hline
  Bandwith & $750$ MHz \\
  \hline
  ADC bits & $12$\\
  \hline
  Tx power & +$13$ dBm\\
  \hline
  \hline
 \end{tabular}}
\caption{The radar system specifications}  
\label{tbl:gest}  
\end{table}






The Ancortek Radar system is used to generate the dataset is a $24$ GHz FMCW radar that has a standalone GUI to control and capture data or can be commanded within a Matlab interface to capture signals. The system has one transmit antenna and two receive antennas (only one was used for the purposes of this dataset). It was set up on a lab bench at the same height as the gesture action. It was then initiated to capture $30$ seconds of data and the candidate repeated the actions numerous times within this window. Afterwards, the raw data was then cut into individual gestures that occurred over the whole period. These individual gesture actions have varying matrix sizes hence a cell data format was used to create a ragged data cube. The data was created by the following flow of processing:
\begin{itemize}
\item De-interleave Channel $1$ $-2$ and I$/$Q samples.
\item Break vector of samples into a $2$D matrix of Chirp vs. Time.
\item FFT samples to covert to range domain. Resulting in a Range vs. Time matrix (RTI)
\item Filter signal such that static targets are suppressed and moving targets are highlighted. This is called MTI filtering in radar signal processing.
\item Extract rows within the RTI that contain the gesture movement and coherently sum these.
\item Generate a Doppler vs. Time $2$D matrix by using a Short Time Fourier Transform on the vector of selected samples.
\item Store the complex samples of the Doppler vs. Time matrix within a larger cell array which is a data cube of the N repeats of the $4$ gestures from each person.
\end{itemize}

Example of a Doppler vs. Time matrix for each gesture can be seen in~ \fig{fourgest}




\begin{figure}
\centering\includegraphics[scale=0.6]{fourgesture.png}
\caption{Doppler vs. Time matrix for each of four gestures ~\cite{dopnet} }
\label{fig:fourgest}
\end{figure}

The waving gesture which has the oscillatory shape and longer duration, whereas the click gesture happens over the shortest time frame (as a click is only a short sharp action). Then the pinch and swipe actions do show some level of similarity which could make them challenging for a classifier.\cite{dopnet}


\tbl{fourgesture} illustrates the number of samples per person. Each sample contains a $2$D matrix of complex-value pixles, the first dimension(Doppler) of all samples'matrices size are the same and equal to $800$, the second dimension of smples'matices(Time) size is not the same for all the samples, the range of the Time dimensions for each gesture are shown in ~\tbl{gestdim}.

\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{%  
 \begin{tabular}{|c|c|c|c|c|c|c|r}
  \hline
  \hline
  Gesture & A & B & C & D & E  & F & Total \\
  \hline
  Wave & 56 & 112 & 85 & 70 & 56 & 87 &  466\\
  \hline
  Pinch & 98 & 116 & 132 & 112 & 98 & 140 & 696\\
  \hline
  Swipe & 64 & 72 & 80 & 71 & 91 & 101 & 479\\
  \hline
  Click & 105 & 105 & 137 & 93 & 144 & 208 & 792\\
  \hline
  \hline
 \end{tabular}%
}
\caption{The number of each gesture's samples per person }  
\label{tbl:fourgesture}  
\end{table}

\begin{table}
\centering\scalebox{0.9}{  
 \begin{tabular}{|c|c|c|c|c|c|c|r}
  \hline
  Gesture & Dimension range \\
  \hline
  \hline
  Wave & 116 - 540\\
  \hline
  Pinch & 60 - 231\\
  \hline
  Swipe & 118 - 480\\
  \hline
  Click & 43 - 211\\
  \hline
  \hline
 \end{tabular}}
\caption{The range of each gesture's Time dimension  }  
\label{tbl:gestdim}  
\end{table}

\subsection{Our Complex-value Datasets}
We have created $2$ complex-value datasets from the Dopnet samples, as \tbl{fourgesture} and \tbl{gestdim} shows wave and swipe gestures samples have similar dimension range and number of samples, the remaining $2$ gestures, pinch and click have similar dimension range and number of samples. Therefore, we chose wave and swipe gesture samples as our complex-$1$binary classifications input dataset and uniformed all the samples dimensions to $800$ $\times$ $540$ by adding zeros wherever the time dimension was less than $540$. Therefore, we have got $945$ complex-value samples in our database. The second complex-value dataset is called complex-$2$ and consists of $1488$ samples, the dimension of the samples in this dataset is $800$ $\times$ $231$, zeros are added wherever the time dimension was less than $231$ we used $80$ percent of the samples in each of the datasets as training and $20$ percent as test samples. So we have:   


\begin{itemize}
\item complex-1 dataset: each sample size is $800$ $\times$ $540$ \\
\item complex-1 dataset: each sample size is $800$ $\times$ $231$ 

\end{itemize}




